Systematic Inequalities in Language Technology Performance across the World's Languages

Natural language processing (NLP) systems have become a central technology in communication, education, medicine, artificial intelligence, and many other domains of research and development. While the performance of NLP methods has grown enormously over the last decade, this progress has been restricted to a minuscule subset of the world's 6,500 languages. We introduce a framework for estimating the global utility of language technologies as revealed in a comprehensive snapshot of recent publications in NLP. Our analyses involve the field at large, but also more in-depth studies on both user-facing technologies (machine translation, language understanding, question answering, text-to-speech synthesis) as well as more linguistic NLP tasks (dependency parsing, morphological inflection). In the process, we (1) quantify disparities in the current state of NLP research, (2) explore some of its associated societal and academic factors, and (3) produce tailored recommendations for evidence-based policy making aimed at promoting more global and equitable language technologies.

==> figures/all_mt_from.tex <==
\begin{figure}
\vspace{-2cm}
\pgfplotstableread[row sep=\\,col sep=&]{
xa & ya \\
0.001 & 0.17 \\
0.002 & 0.24 \\
0.003 & 0.30 \\
0.004 & 0.35 \\
0.005 & 0.39 \\
0.006 & 0.43 \\
0.007 & 0.47 \\
0.008 & 0.50 \\
0.009 & 0.53 \\
0.01 & 0.55 \\
0.011 & 0.56 \\
0.012 & 0.58 \\
0.013 & 0.59 \\
0.014 & 0.60 \\
0.015 & 0.62 \\
0.016 & 0.63 \\
0.017 & 0.64 \\
0.018 & 0.65 \\
0.019 & 0.66 \\
0.02 & 0.67 \\
0.021 & 0.68 \\
0.022 & 0.69 \\
0.023 & 0.70 \\
0.024 & 0.71 \\
0.025 & 0.72 \\
0.026 & 0.73 \\
0.027 & 0.74 \\
0.028 & 0.75 \\
0.029 & 0.76 \\
0.031 & 0.77 \\
0.032 & 0.78 \\
0.034 & 0.79 \\
0.036 & 0.80 \\
0.038 & 0.81 \\
0.04 & 0.82 \\
0.042 & 0.83 \\
0.044 & 0.84 \\
0.046 & 0.85 \\
0.049 & 0.86 \\
0.052 & 0.87 \\
0.055 & 0.88 \\
0.058 & 0.89 \\
0.062 & 0.90 \\
0.066 & 0.91 \\
0.071 & 0.92 \\
0.078 & 0.93 \\
0.085 & 0.94 \\
0.094 & 0.95 \\
0.105 & 0.96 \\
0.119 & 0.97 \\
0.138 & 0.98 \\
0.174 & 0.99 \\
0.267 & 1.00 \\
1 & 1\\
}\fdata
\pgfplotstableread[row sep=\\,col sep=&]{
lang & m & gini \\
afr & 0.234 & 0.498 \\
amh & 0.107 & 0.497 \\
ara & 0.158 & 0.522 \\
asm & 0.250 & 0.497 \\
aze & 0.118 & 0.497 \\
bel & 0.121 & 0.496 \\
ben & 0.106 & 0.519 \\
bos & 0.151 & 0.496 \\
bre & 0.096 & 0.496 \\
bul & 0.175 & 0.496 \\
cat & 0.176 & 0.497 \\
ces & 0.162 & 0.497 \\
cmn & 0.153 & 0.618 \\
cym & 0.231 & 0.496 \\
dan & 0.191 & 0.496 \\
deu & 0.259 & 0.504 \\
ell & 0.168 & 0.497 \\
eng & 0.286 & 0.515 \\
epo & 0.173 & 0.496 \\
est & 0.147 & 0.496 \\
eus & 0.125 & 0.496 \\
fas & 0.118 & 0.499 \\
fin & 0.157 & 0.496 \\
fra & 0.232 & 0.509 \\
fry & 0.194 & 0.496 \\
gla & 0.298 & 0.495 \\
gle & 0.264 & 0.496 \\
glg & 0.165 & 0.529 \\
guj & 0.281 & 0.496 \\
hau & 0.107 & 0.499 \\
heb & 0.164 & 0.496 \\
hin & 0.171 & 0.524 \\
hrv & 0.240 & 0.496 \\
hun & 0.128 & 0.496 \\
hye & 0.086 & 0.495 \\
ibo & 0.243 & 0.498 \\
ind & 0.157 & 0.516 \\
isl & 0.111 & 0.496 \\
ita & 0.183 & 0.504 \\
jpn & 0.130 & 0.509 \\
kan & 0.170 & 0.498 \\
kat & 0.110 & 0.496 \\
kaz & 0.145 & 0.496 \\
khm & 0.143 & 0.497 \\
kin & 0.108 & 0.496 \\
kir & 0.167 & 0.496 \\
kor & 0.078 & 0.499 \\
kur & 0.110 & 0.496 \\
lav & 0.211 & 0.496 \\
lim & 0.177 & 0.496 \\
lit & 0.194 & 0.496 \\
mal & 0.090 & 0.492 \\
mar & 0.198 & 0.497 \\
mkd & 0.158 & 0.496 \\
mlg & 0.128 & 0.497 \\
mlt & 0.282 & 0.496 \\
mon & 0.034 & 0.495 \\
msa & 0.140 & 0.501 \\
mya & 0.067 & 0.498 \\
nep & 0.245 & 0.506 \\
nld & 0.173 & 0.497 \\
nnp & 0.180 & 0.495 \\
nob & 0.190 & 0.496 \\
oci & 0.092 & 0.495 \\
ori & 0.133 & 0.498 \\
orm & 0.088 & 0.495 \\
pan & 0.203 & 0.499 \\
pol & 0.122 & 0.498 \\
por & 0.227 & 0.574 \\
pus & 0.197 & 0.500 \\
ron & 0.202 & 0.498 \\
rus & 0.187 & 0.509 \\
sin & 0.108 & 0.496 \\
slk & 0.178 & 0.496 \\
slv & 0.306 & 0.496 \\
sme & 0.070 & 0.495 \\
som & 0.101 & 0.496 \\
spa & 0.202 & 0.575 \\
sqi & 0.194 & 0.496 \\
srp & 0.250 & 0.496 \\
swa & 0.149 & 0.497 \\
swe & 0.169 & 0.497 \\
tam & 0.124 & 0.496 \\
tat & 0.081 & 0.496 \\
tel & 0.161 & 0.503 \\
tgj & 0.106 & 0.495 \\
tgl & 0.156 & 0.498 \\
tha & 0.100 & 0.498 \\
tir & 0.088 & 0.495 \\
tuk & 0.243 & 0.496 \\
tur & 0.141 & 0.501 \\
uig & 0.084 & 0.496 \\
ukr & 0.129 & 0.502 \\
urd & 0.098 & 0.504 \\
uzb & 0.087 & 0.497 \\
vie & 0.126 & 0.499 \\
wln & 0.162 & 0.496 \\
xho & 0.113 & 0.496 \\
yid & 0.157 & 0.496 \\
zul & 0.239 & 0.498 \\
}\mtdata
\centering
\newcommand\dottedcircle{\raisebox{-.1em}{\tikz \draw [line cap=round, line width=0.2ex, dash pattern=on 0pt off 0.5ex] (0,0) circle [radius=0.79ex];}}
\begin{tikzpicture}
    [trim left=15cm,
     trim right=0cm,
     mycirc/.style={circle,solid,fill=white,draw=black,inner sep=0pt,minimum size=4pt},
     mycirctwo/.style={circle,solid,fill=black,draw=black,inner sep=0pt,minimum size=4pt},
     every pin/.style = {%pin distance=2mm, 
                font=\scriptsize, inner sep=1pt},
    PNtwo/.style args = {#1/#2}{% Pin Node
    mycirctwo, pin=#1:#2}
     ]
    \begin{axis}[
    title={},
    width=12cm,
    height=12cm,
    ymin=-1,ymax=1.5,xmin=-1,xmax=1.5,
    ytick={0,1},xtick={0,1},
    ymajorgrids=false,
    yminorgrids=false,
    every axis plot post/.style={/pgf/number format/fixed},        
    axis x line*=bottom,
    axis y line*=left,
    hide y axis,
    hide x axis,
    xtick style={draw=none},
    ytick style={draw=none},
    %xtick label style={draw=none},
    %axis x line style={draw=none},
    %ymode=log,
    ]
    \path[name path=axis1] (axis cs:0,0) -- (axis cs:1,0);
    \path[name path=axis2] (axis cs:0,1) -- (axis cs:1,1);
    \draw [->] (0,0) -- (1.05,0) node [midway, below, text width=3cm, align=center] {\small Demographic Fairness};
    \draw [->] (0,0) -- (0,1.05) node [midway, above, rotate=90,text width=3cm, align=center] {\small Linguistic Fairness};
    \node[mycirc, label=above:{Ideal}] at (axis cs:1,1) {};
    \node[label=below:{0}] at (axis cs:0,0.05) {};
    \node[label=below:{1}] at (axis cs:1,0) {};
    \node[label=left:{1}] at (axis cs:0,1) {};
    \addplot [name path=f, mark=none, black] table[x=ya,y=xa]{\fdata};
    %\addplot[name path=f, domain=0:1,black] {x^8};
    \addplot [thick,color=gray, fill=gray, fill opacity=0.1]
    fill between[of=f and axis1,soft clip={domain=0:1},];
    \addplot [name path=g, mark=none, black] table[x=xa,y=ya]{\fdata};
    %\addplot[name path=g, domain=0:1,black] {x^.2};
    \addplot [thick,color=gray, fill=gray, fill opacity=0.1,]
    fill between[of=axis2 and g,soft clip={domain=0:1},];
    % My stuff
    \node[mycirctwo] table[x=m,y=gini]{\mtdata};
    %\node[mycirctwo] at (axis cs:0.206,0.012) {}; 
    %\node[mycirctwo, pin={[pin distance=4mm]90:{\small MT$_{x\rightarrow\text{eng}}$}}] at (axis cs:0.35,0.26) {}; 
    \end{axis}
\end{tikzpicture}
\vspace{-3.5cm}
\label{fig:mt}
\caption{MT }
\end{figure}

==> figures/overview.tex <==
\sidecaptionvpos{figure}{c}
\begin{SCfigure*}[][t]
%\begin{figure}
\pgfplotstableread[row sep=\\,col sep=&]{
xa & ya \\
0.001 & 0.17 \\
0.002 & 0.24 \\
0.003 & 0.30 \\
0.004 & 0.35 \\
0.005 & 0.39 \\
0.006 & 0.43 \\
0.007 & 0.47 \\
0.008 & 0.50 \\
0.009 & 0.53 \\
0.01 & 0.55 \\
0.011 & 0.56 \\
0.012 & 0.58 \\
0.013 & 0.59 \\
0.014 & 0.60 \\
0.015 & 0.62 \\
0.016 & 0.63 \\
0.017 & 0.64 \\
0.018 & 0.65 \\
0.019 & 0.66 \\
0.02 & 0.67 \\
0.021 & 0.68 \\
0.022 & 0.69 \\
0.023 & 0.70 \\
0.024 & 0.71 \\
0.025 & 0.72 \\
0.026 & 0.73 \\
0.027 & 0.74 \\
0.028 & 0.75 \\
0.029 & 0.76 \\
0.031 & 0.77 \\
0.032 & 0.78 \\
0.034 & 0.79 \\
0.036 & 0.80 \\
0.038 & 0.81 \\
0.04 & 0.82 \\
0.042 & 0.83 \\
0.044 & 0.84 \\
0.046 & 0.85 \\
0.049 & 0.86 \\
0.052 & 0.87 \\
0.055 & 0.88 \\
0.058 & 0.89 \\
0.062 & 0.90 \\
0.066 & 0.91 \\
0.071 & 0.92 \\
0.078 & 0.93 \\
0.085 & 0.94 \\
0.094 & 0.95 \\
0.105 & 0.96 \\
0.119 & 0.97 \\
0.138 & 0.98 \\
0.174 & 0.99 \\
0.267 & 1.00 \\
1 & 1\\
}\fdata

\pgfplotstableread[row sep=\\,col sep=&]{
xa & ya \\
0.18 & 0.00 \\ 
0.26 & 0.01 \\ 
0.32 & 0.01 \\ 
0.36 & 0.01 \\ 
0.41 & 0.01 \\ 
0.45 & 0.02 \\ 
0.48 & 0.02 \\ 
0.50 & 0.02 \\ 
0.53 & 0.02 \\ 
0.55 & 0.03 \\ 
0.56 & 0.03 \\ 
0.57 & 0.03 \\ 
0.59 & 0.03 \\ 
0.60 & 0.04 \\ 
0.61 & 0.04 \\ 
0.62 & 0.04 \\ 
0.64 & 0.04 \\ 
0.65 & 0.05 \\ 
0.66 & 0.05 \\ 
0.67 & 0.05 \\ 
0.68 & 0.05 \\ 
0.69 & 0.05 \\ 
0.70 & 0.06 \\ 
0.71 & 0.06 \\ 
0.72 & 0.06 \\ 
0.73 & 0.06 \\ 
0.73 & 0.07 \\ 
0.74 & 0.07 \\ 
0.75 & 0.07 \\ 
0.76 & 0.07 \\ 
0.76 & 0.08 \\ 
0.77 & 0.08 \\ 
0.78 & 0.08 \\ 
0.79 & 0.08 \\ 
0.79 & 0.09 \\ 
0.80 & 0.09 \\ 
0.81 & 0.09 \\ 
0.82 & 0.10 \\ 
0.83 & 0.10 \\ 
0.84 & 0.11 \\ 
0.85 & 0.11 \\ 
0.86 & 0.12 \\ 
0.87 & 0.12 \\ 
0.87 & 0.13 \\ 
0.88 & 0.13 \\ 
0.88 & 0.14 \\ 
0.89 & 0.14 \\ 
0.90 & 0.15 \\ 
0.91 & 0.16 \\ 
0.91 & 0.17 \\ 
0.92 & 0.17 \\ 
0.92 & 0.18 \\ 
0.93 & 0.18 \\ 
0.93 & 0.19 \\ 
0.94 & 0.20 \\ 
0.94 & 0.21 \\ 
0.95 & 0.21 \\ 
0.95 & 0.22 \\ 
0.95 & 0.23 \\ 
0.96 & 0.23 \\ 
0.96 & 0.24 \\ 
0.96 & 0.25 \\ 
0.97 & 0.26 \\ 
0.97 & 0.27 \\ 
0.97 & 0.28 \\ 
0.97 & 0.29 \\ 
0.98 & 0.29 \\ 
0.98 & 0.30 \\ 
0.98 & 0.31 \\ 
0.98 & 0.32 \\ 
0.98 & 0.33 \\ 
0.98 & 0.34 \\ 
0.98 & 0.35 \\ 
0.99 & 0.35 \\ 
0.99 & 0.36 \\ 
0.99 & 0.37 \\ 
0.99 & 0.38 \\ 
0.99 & 0.39 \\ 
0.99 & 0.40 \\ 
0.99 & 0.41 \\ 
0.99 & 0.42 \\ 
0.99 & 0.43 \\ 
0.99 & 0.44 \\ 
0.99 & 0.45 \\ 
0.99 & 0.46 \\ 
0.99 & 0.47 \\ 
0.99 & 0.48 \\ 
1.00 & 0.49 \\ 
1.00 & 0.50 \\ 
1.00 & 0.51 \\ 
1.00 & 0.52 \\ 
1.00 & 0.53 \\ 
1.00 & 0.54 \\ 
1.00 & 0.55 \\ 
1.00 & 0.56 \\ 
1.00 & 0.57 \\ 
1.00 & 0.58 \\ 
1.00 & 0.59 \\ 
1.00 & 0.60 \\ 
1.00 & 0.61 \\ 
1.00 & 0.62 \\ 
1.00 & 0.63 \\ 
1.00 & 0.64 \\ 
1.00 & 0.65 \\ 
1.00 & 0.66 \\ 
1.00 & 0.67 \\ 
1.00 & 0.68 \\ 
1.00 & 0.69 \\ 
1.00 & 0.70 \\ 
1.00 & 0.71 \\ 
1.00 & 0.72 \\ 
1.00 & 0.73 \\ 
1.00 & 0.74 \\ 
1.00 & 0.75 \\ 
1.00 & 0.76 \\ 
1.00 & 0.77 \\ 
1.00 & 0.78 \\ 
1.00 & 0.79 \\ 
1.00 & 0.80 \\ 
1.00 & 0.81 \\ 
1.00 & 0.82 \\ 
1.00 & 0.83 \\ 
1.00 & 0.84 \\ 
1.00 & 0.85 \\ 
1.00 & 0.86 \\ 
1.00 & 0.87 \\ 
1.00 & 0.88 \\ 
1.00 & 0.89 \\ 
1.00 & 0.90 \\ 
1.00 & 0.91 \\ 
1.00 & 0.92 \\ 
1.00 & 0.93 \\ 
1.00 & 0.94 \\ 
1.00 & 0.95 \\ 
1.00 & 0.96 \\ 
1.00 & 0.97 \\ 
1.00 & 0.98 \\ 
1.00 & 0.99 \\ 
1.00 & 1.00 \\ 
}\cfdataone

\pgfplotstableread[row sep=\\,col sep=&]{
xa & ya \\
0.15 & 0.00 \\ 
0.20 & 0.00 \\ 
0.26 & 0.01 \\ 
0.29 & 0.01 \\ 
0.33 & 0.01 \\ 
0.36 & 0.01 \\ 
0.38 & 0.02 \\ 
0.40 & 0.02 \\ 
0.42 & 0.02 \\ 
0.44 & 0.02 \\ 
0.45 & 0.02 \\ 
0.46 & 0.03 \\ 
0.47 & 0.03 \\ 
0.48 & 0.03 \\ 
0.49 & 0.03 \\ 
0.50 & 0.03 \\ 
0.51 & 0.03 \\ 
0.52 & 0.04 \\ 
0.53 & 0.04 \\ 
0.54 & 0.04 \\ 
0.55 & 0.04 \\ 
0.56 & 0.05 \\ 
0.57 & 0.05 \\ 
0.58 & 0.05 \\ 
0.59 & 0.05 \\ 
0.60 & 0.06 \\ 
0.61 & 0.06 \\ 
0.62 & 0.06 \\ 
0.62 & 0.07 \\ 
0.63 & 0.07 \\ 
0.64 & 0.07 \\ 
0.65 & 0.07 \\ 
0.65 & 0.08 \\ 
0.66 & 0.08 \\ 
0.67 & 0.08 \\ 
0.67 & 0.09 \\ 
0.68 & 0.09 \\ 
0.69 & 0.09 \\ 
0.69 & 0.10 \\ 
0.70 & 0.10 \\ 
0.70 & 0.11 \\ 
0.71 & 0.11 \\ 
0.72 & 0.12 \\ 
0.73 & 0.12 \\ 
0.73 & 0.13 \\ 
0.73 & 0.14 \\ 
0.74 & 0.14 \\ 
0.74 & 0.15 \\ 
0.75 & 0.15 \\ 
0.75 & 0.16 \\ 
0.75 & 0.17 \\ 
0.76 & 0.17 \\ 
0.76 & 0.18 \\ 
0.76 & 0.19 \\ 
0.77 & 0.19 \\ 
0.77 & 0.20 \\ 
0.77 & 0.21 \\ 
0.78 & 0.21 \\ 
0.78 & 0.22 \\ 
0.78 & 0.23 \\ 
0.78 & 0.24 \\ 
0.78 & 0.25 \\ 
0.78 & 0.26 \\ 
0.79 & 0.26 \\ 
0.79 & 0.27 \\ 
0.79 & 0.28 \\ 
0.79 & 0.29 \\ 
0.79 & 0.30 \\ 
0.79 & 0.31 \\ 
0.79 & 0.32 \\ 
0.79 & 0.33 \\ 
0.79 & 0.34 \\ 
0.79 & 0.35 \\ 
0.79 & 0.36 \\ 
0.80 & 0.36 \\ 
0.80 & 0.37 \\ 
0.80 & 0.38 \\ 
0.80 & 0.39 \\ 
0.80 & 0.40 \\ 
0.80 & 0.41 \\ 
0.80 & 0.42 \\ 
0.80 & 0.43 \\ 
0.80 & 0.44 \\ 
0.80 & 0.45 \\ 
0.80 & 0.46 \\ 
0.80 & 0.47 \\ 
0.80 & 0.48 \\ 
0.80 & 0.49 \\ 
0.80 & 0.50 \\ 
0.80 & 0.51 \\ 
0.80 & 0.52 \\ 
0.80 & 0.53 \\ 
0.80 & 0.54 \\ 
0.80 & 0.55 \\ 
0.80 & 0.56 \\ 
0.80 & 0.57 \\ 
0.80 & 0.58 \\ 
0.80 & 0.59 \\ 
0.80 & 0.60 \\ 
0.80 & 0.61 \\ 
0.80 & 0.62 \\ 
0.80 & 0.63 \\ 
0.80 & 0.64 \\ 
0.80 & 0.65 \\ 
0.80 & 0.66 \\ 
0.80 & 0.67 \\ 
0.80 & 0.68 \\ 
0.80 & 0.69 \\ 
0.80 & 0.70 \\ 
0.80 & 0.71 \\ 
0.80 & 0.72 \\ 
0.80 & 0.73 \\ 
0.80 & 0.74 \\ 
0.80 & 0.75 \\ 
0.80 & 0.76 \\ 
0.80 & 0.77 \\ 
0.80 & 0.78 \\ 
0.80 & 0.79 \\ 
0.80 & 0.80 \\ 
}\cfdatatwo

\pgfplotstableread[row sep=\\,col sep=&]{
xa & ya \\
0 & 1 \\
1 & 1\\
}\dummydata
\centering
\newcommand\dottedcircle{\raisebox{-.1em}{\tikz \draw [line cap=round, line width=0.2ex, dash pattern=on 0pt off 0.5ex] (0,0) circle [radius=0.79ex];}}
%\resizebox{.03\textwidth}{!}{%
\vspace{-2cm}
\begin{tikzpicture}
    [trim left=0cm,
     trim right=9cm,
     scale=1,
     mycirc/.style={circle,solid,fill=white,draw=black,inner sep=0pt,minimum size=4pt},
     mycirctwo/.style={circle,solid,fill=black,draw=black,inner sep=0pt,minimum size=4pt},
     mydiamond/.style={diamond,solid,fill=white,draw=black,inner sep=0pt,minimum size=4pt},
     graysquare/.style={square*,solid,fill=gray!0.1,draw=gray!0.1,inner sep=0pt,minimum size=4pt},
     every pin/.style = {%pin distance=2mm, 
                font=\scriptsize, inner sep=1pt},
    PNtwo/.style args = {#1/#2}{mycirctwo, pin=#1:#2}
     ]
    \begin{axis}[
    title={},
    width=12cm,
    height=12cm,
    xshift=-4cm,
    yshift=1cm,
    ymin=-1,ymax=1.5,xmin=-1,xmax=1.5,
    ytick={0,1},xtick={0,1},
    ymajorgrids=false,
    yminorgrids=false,
    every axis plot post/.style={/pgf/number format/fixed},        
    axis x line*=bottom,
    axis y line*=left,
    hide y axis,
    hide x axis,
    xtick style={draw=none},
    ytick style={draw=none},
    %xtick label style={draw=none},
    %axis x line style={draw=none},
    %ymode=log,
    ]
    \path[name path=axis1] (axis cs:0,0) -- (axis cs:1,0);
    \path[name path=axis2] (axis cs:0,1) -- (axis cs:1,1);
    \draw [->] (0,0) -- (1.05,0) node [midway, below=1.5mm, text width=3cm, align=center] {{\small Demographic Fairness \\ \small ($\tau$=1)}};
    \draw [->] (0,0) -- (0,1.05) node [midway, above, rotate=90,text width=3cm, align=center] {\small Linguistic Fairness \\ \small ($\tau$=0)};
    \node[mycirc, label=above:{Ideal}] at (axis cs:1,1) {};
    \node[label=below:{0}] at (axis cs:0,0.05) {};
    \node[label=below:{1}] at (axis cs:1,0) {};
    \node[label=left:{1}] at (axis cs:0,1) {};
    %\node[label=left:{0.1}] at (axis cs:0,0.666) {};
    %\addplot [name path=h, mark=none, white] table[x=xa,y=ya]{\dummydata};
    %\addplot [thick,color=gray, fill=gray, fill opacity=0.1] fill between[of=h and axis1,soft clip={domain=0:1},];
    \addplot [name path=g, mark=none, black] table[x=xa,y=ya]{\fdata};
    \addplot [thick,color=white,fill=white] fill between[of=g and axis1,soft clip={domain=0:1},];
    \addplot [name path=f, mark=none, black] table[x=ya,y=xa]{\fdata};
    \addplot [thick,color=gray, fill=gray, fill opacity=0.1] fill between[of=f and axis1,soft clip={domain=0:1},];
    \addplot [thick,color=gray, fill=gray, fill opacity=0.1] fill between[of=axis2 and g,soft clip={domain=0:1},];
    % My stuff
    % Counterfactual Curve with going to next language after accuracy 1 in previous language, languages in demographic order
    \addplot [name path=cf, mark=none, red] table[x=xa,y=ya]{\cfdataone};
    % As above, but accuracy 0.9 per language
    \addplot [name path=cf, mark=none, blue] table[x=xa,y=ya]{\cfdatatwo};
    % Inflection
    \node[mycirctwo, pin={[pin distance=2mm]45:{\small Inflection}}] at (axis cs:0.564,0.13) {}; 
    % DEP
    \node[mycirctwo, pin={[pin distance=2mm]90:{\small DEP}}] at (axis cs:0.473,0.052) {}; 
    % MT Eng to x
    \node[mycirctwo] at (axis cs:0.326,0.042) {};
    % MT x to Eng
    \node[mycirctwo] at (axis cs:0.35,0.052) {}; 
    % Papers
    \node[mydiamond] at (axis cs:0.101,0.005) {}; 
    %NLI
    \node[mycirctwo] at (axis cs:0.359,0.0132) {}; 
    %QA
    \node[mycirctwo] at (axis cs:0.46,0.011) {}; 
    %MT X to all
    \node[mycirctwo] at (axis cs:0.382,0.049) {}; 
    %MT all to X
    \node[mycirctwo] at (axis cs:0.340,0.0386) {}; 
    % Synthesis
    \node[mycirctwo, pin={[pin distance=2mm]90:{\small Synthesis}}] at (axis cs:0.27,0.32) {}; 
    % Counterfactuals
    \node[mydiamond, pin={[pin distance=4mm]90:{\small \textsc{cf-eng}}}] at (axis cs:0.063,0.002) {}; 
    \node[mydiamond, pin={[pin distance=1mm]90:{\small \textsc{cf-cmn}}}] at (axis cs:0.1815,0.003) {}; 
    \node[mydiamond, pin={[pin distance=2mm]10:{\small \textsc{cf-t50}}}] at (axis cs:0.479,0.019) {}; 
    \node[mydiamond, pin={[pin distance=1mm]90:{\small \textsc{cf-b50}}}] at (axis cs:0.521,0.98) {}; 
    \node[mydiamond, pin={[pin distance=1mm]95:{\small \textsc{cf-linear}}}] at (axis cs:0.96,0.59) {}; 
    %
    % Zoom in
    \draw[gray,opacity=0.6] (0,0.1) -- (0.5,0.1); 
    \draw[gray,opacity=0.6] (0.5,0) -- (0.5,0.1); 
    \end{axis}
    \begin{axis}[
    xshift=-.7cm,
    yshift=1.5cm,
    title={},
    %scale=1.2,
    width=12cm,
    height=9cm,
    ymin=-1,ymax=1,xmin=-1,xmax=0.75,
    ytick={0,1},xtick={0,1},
    ymajorgrids=false,
    yminorgrids=false,
    every axis plot post/.style={/pgf/number format/fixed},        
    axis x line*=bottom,
    axis y line*=left,
    hide y axis,
    hide x axis,
    xtick style={draw=none},
    ytick style={draw=none},
    %xtick label style={draw=none},
    %axis x line style={draw=none},
    %ymode=log,
    ]
    \path[name path=axis1b] (axis cs:0,0) -- (axis cs:0.65,0);
    \path[name path=axis2b] (axis cs:0,0.65) -- (axis cs:0.5,0.65);
    \draw (0,0) -- (0.6,0);
    \draw (0,0.5) -- (0.6,0.5);
    \draw (0.6,0) -- (0.6,0.5);
    \draw (0,0) -- (0,0.5);
    \node[label=below:{0}] at (axis cs:0,0.03) {};
    \node[label=below:{0.5}] at (axis cs:0.5,0.03) {};
    \node[label=left:{0.1}] at (axis cs:0.03,0.5) {};
    \addplot[name path=f, domain=0:0.6,black] {x^5};
    \addplot [thick,color=gray, fill=gray, fill opacity=0.1]
    fill between[of=f and axis1b,soft clip={domain=0:0.6},];
    %\addplot[name path=g, domain=0:0.037,black] {x^.16};
    %\addplot [thick,color=gray, fill=gray, fill opacity=0.1,]
    %fill between[of=axis2b and g,soft clip={domain=0:0.037},];
    % My stuff
    %\node[PNtwo=-35/{\small DEP}] at (axis cs:0.473,0.052) {}; 
    %\node[mycirctwo, pin={[pin distance=2mm]0:{\small DEP}}] at (axis cs:0.473,0.26) {}; 
    %\node[PNtwo=-35/{\small MT$_{eng\rightarrow x}$}] at (axis cs:0.326,0.042) {};
    \node[mycirctwo, pin={[pin distance=2mm]130:{\small MT$_{\text{eng}\rightarrow x}$}}] at (axis cs:0.326,0.21) {};
    %\node[PNtwo=90/{\small MT$_{x\rightarrow eng}$}] at (axis cs:0.35,0.052) {}; 
    \node[mycirctwo, pin={[pin distance=4mm]90:{\small MT$_{x\rightarrow\text{eng}}$}}] at (axis cs:0.35,0.26) {}; 
    %x->all
    \node[mycirctwo, pin={[pin distance=2mm]45:{\small MT$_{x\rightarrow\text{all}}$}}] at (axis cs:0.382,0.245) {}; 
    %all->x
    \node[mycirctwo, pin={[pin distance=2mm]0:{\small MT$_{\text{all}\rightarrow x}$}}] at (axis cs:0.340,0.19) {}; 
    %\node[PNtwo=0/{\small Papers}] at (axis cs:0.101,0.005) {}; 
    \node[mydiamond, pin={[pin distance=1mm]135:{\small MT Papers}}] at (axis cs:0.101,0.025) {}; 
    \node[mycirctwo, pin={[pin distance=1mm]120:{\small NLI}}] at (axis cs:0.359,0.0132) {}; 
    \node[mycirctwo, pin={[pin distance=1mm]90:{\small QA}}] at (axis cs:0.46,0.021) {}; 
    \node[mydiamond, ] at (axis cs:0.063,0.002) {}; 
    \node[mydiamond, ] at (axis cs:0.1815,0.003) {}; 
    %\node[mydiamond, pin={[pin distance=4mm]90:{\small \textsc{cf-eng}}}] at (axis cs:0.063,0.002) {}; 
    %\node[mydiamond, pin={[pin distance=1mm]90:{\small \textsc{cf-cmn}}}] at (axis cs:0.1815,0.003) {}; 
    %\node[mydiamond, pin={[pin distance=2mm]0:{\small \textsc{cf-t50}}}] at (axis cs:0.479,0.019) {}; 

    %\node[PNtwo=0/{\small Synthesis}] at (axis cs:0.27,0.32) {}; 
    %\node[PNtwo=0/{\small Synthesis}] at (axis cs:0.27,0.72) {}; 
    \end{axis}
    \iffalse
    \begin{axis}[
    xshift=-.7cm,
    yshift=4.1cm,
    title={},
    %scale=1.2,
    width=12cm,
    height=9cm,
    ymin=-1,ymax=1,xmin=-1,xmax=0.75,
    ytick={0,1},xtick={0,1},
    ymajorgrids=false,
    yminorgrids=false,
    every axis plot post/.style={/pgf/number format/fixed},        
    axis x line*=bottom,
    axis y line*=left,
    hide y axis,
    hide x axis,
    xtick style={draw=none},
    ytick style={draw=none},
    %xtick label style={draw=none},
    %axis x line style={draw=none},
    %ymode=log,
    ]
    \path[name path=axis1b] (axis cs:0,0) -- (axis cs:0.65,0);
    \path[name path=axis2b] (axis cs:0,0.65) -- (axis cs:0.5,0.65);
    %\draw [->] (0,0) -- (0.55,0) node {{\small Demographic Fairness \\ \small ($\tau$=1)}};
    \draw (0,0) -- (0.6,0);
    \draw (0,0.5) -- (0.6,0.5);
    \draw (0.6,0) -- (0.6,0.5);
    %\draw [->] (0,0) -- (0,0.55) node [midway, above, rotate=90,text width=3cm, align=center] {\small Linguistic Fairness \\ \small ($\tau$=0)};
    \draw (0,0) -- (0,0.5);
    %\node[mycirc, label=above:{Ideal}] at (axis cs:1,1) {};
    \node[label={Progression on}] at (axis cs:0.22,0.34) {};
    \node[label={Inflection}] at (axis cs:0.16,0.24) {};
    \node[label=below:{0}] at (axis cs:0,0.03) {};
    \node[label=below:{0.5}] at (axis cs:0.5,0.03) {};
    \node[label=left:{0.1}] at (axis cs:0.03,0.5) {};
    \addplot[name path=f, domain=0:0.6,black] {x^5};
    \addplot [thick,color=gray, fill=gray, fill opacity=0.1]
    fill between[of=f and axis1b,soft clip={domain=0:0.6},];
    %\addplot[name path=g, domain=0:0.037,black] {x^.16};
    %\addplot [thick,color=gray, fill=gray, fill opacity=0.1,]
    %fill between[of=axis2b and g,soft clip={domain=0:0.037},];
    % My stuff
    \node[mycirctwo, pin={[pin distance=2mm]90:{\small 2020}}] at (axis cs:0.564,0.26) {}; 
    \node[mycirctwo, pin={[pin distance=2mm]30:{\small 2019}}] at (axis cs:0.54,0.18) {};
    \node[mycirctwo, pin={[pin distance=2mm]150:{\small 2018}}] at (axis cs:0.54,0.16) {};
    \node[mycirctwo, pin={[pin distance=2mm]180:{\small 2017}}] at (axis cs:0.497,0.11) {};
    \node[mycirctwo, pin={[pin distance=2mm]90:{\small 2016}}] at (axis cs:0.16,0.03) {};
    \end{axis}
    \fi
    %\node[mycirctwo,label=right:{: NLP tasks}] at (0.2,10) {};
    %\node[mydiamond,label=right:{: Other measures}] at (2.3,10.05) {};
    %\node[label=right:{\textcolor{gray}{$\blacksquare$}\ : Impossible values}] at (5.1,10) {};
    \node[mycirctwo,label=right:{: NLP tasks}] at (5.5,9) {};
    \node[mydiamond,label=right:{: Other measures}] at (5.5,8.6) {};
    \node[label=right:{\textcolor{gray}{$\blacksquare$}\ : Impossible values}] at (5.1,8.2) {};
\end{tikzpicture}
%}
\vspace{-2.5cm}
\caption{Overview of the current state of NLP technologies along the two fairness axes we define in our framework (left); a point to the right of the $x$ axis represents systems that perform well over the largest number of users, and a point at the top of the $y$ axis represents systems that perform well over a large number of languages. We show a zoomed-in version using using $\mathcal{L}=1000$ languages instead of 6500 for visualization purposes.% at the bottom right. 
Most tasks are far from the ideal of being useful for all users and linguistic communities; they are, instead, close to the counter-factual scenario where the utility is linearly distributed only to the top 50\% of the languages with the largest population (\textsc{cf-t50}). Speech synthesis is the only technology we study where research is more linguistically than demographically fair.% The framework allows for tracking the historical progression in a task, which we show for morphological inflection (top right).
%\an{How should we show the counterfactual curves?}
%\gn{Should remove ``Fairness'' in the axis titles. Should make $\mathcal{L}$ to cover all languages. Remove Chinese from plot. Change to squared coordinates. (Damian will help)}
}
\label{fig:overview}
%\end{figure}
\end{SCfigure*}

==> newfigures/historical.tex <==
\begin{figure}[t]
%\begin{figure}
\pgfplotstableread[row sep=\\,col sep=&]{
xa & ya \\
0.001 & 0.17 \\
0.002 & 0.24 \\
0.003 & 0.30 \\
0.004 & 0.35 \\
0.005 & 0.39 \\
0.006 & 0.43 \\
0.007 & 0.47 \\
0.008 & 0.50 \\
0.009 & 0.53 \\
0.01 & 0.55 \\
0.011 & 0.56 \\
0.012 & 0.58 \\
0.013 & 0.59 \\
0.014 & 0.60 \\
0.015 & 0.62 \\
0.016 & 0.63 \\
0.017 & 0.64 \\
0.018 & 0.65 \\
0.019 & 0.66 \\
0.02 & 0.67 \\
0.021 & 0.68 \\
0.022 & 0.69 \\
0.023 & 0.70 \\
0.024 & 0.71 \\
0.025 & 0.72 \\
0.026 & 0.73 \\
0.027 & 0.74 \\
0.028 & 0.75 \\
0.029 & 0.76 \\
0.031 & 0.77 \\
0.032 & 0.78 \\
0.034 & 0.79 \\
0.036 & 0.80 \\
0.038 & 0.81 \\
0.04 & 0.82 \\
0.042 & 0.83 \\
0.044 & 0.84 \\
0.046 & 0.85 \\
0.049 & 0.86 \\
0.052 & 0.87 \\
0.055 & 0.88 \\
0.058 & 0.89 \\
0.062 & 0.90 \\
0.066 & 0.91 \\
0.071 & 0.92 \\
0.078 & 0.93 \\
0.085 & 0.94 \\
0.094 & 0.95 \\
0.105 & 0.96 \\
0.119 & 0.97 \\
0.138 & 0.98 \\
0.174 & 0.99 \\
0.267 & 1.00 \\
1 & 1\\
}\fdata

\pgfplotstableread[row sep=\\,col sep=&]{
xa & ya \\
0.18 & 0.00 \\ 
0.26 & 0.01 \\ 
0.32 & 0.01 \\ 
0.36 & 0.01 \\ 
0.41 & 0.01 \\ 
0.45 & 0.02 \\ 
0.48 & 0.02 \\ 
0.50 & 0.02 \\ 
0.53 & 0.02 \\ 
0.55 & 0.03 \\ 
0.56 & 0.03 \\ 
0.57 & 0.03 \\ 
0.59 & 0.03 \\ 
0.60 & 0.04 \\ 
0.61 & 0.04 \\ 
0.62 & 0.04 \\ 
0.64 & 0.04 \\ 
0.65 & 0.05 \\ 
0.66 & 0.05 \\ 
0.67 & 0.05 \\ 
0.68 & 0.05 \\ 
0.69 & 0.05 \\ 
0.70 & 0.06 \\ 
0.71 & 0.06 \\ 
0.72 & 0.06 \\ 
0.73 & 0.06 \\ 
0.73 & 0.07 \\ 
0.74 & 0.07 \\ 
0.75 & 0.07 \\ 
0.76 & 0.07 \\ 
0.76 & 0.08 \\ 
0.77 & 0.08 \\ 
0.78 & 0.08 \\ 
0.79 & 0.08 \\ 
0.79 & 0.09 \\ 
0.80 & 0.09 \\ 
0.81 & 0.09 \\ 
0.82 & 0.10 \\ 
0.83 & 0.10 \\ 
0.84 & 0.11 \\ 
0.85 & 0.11 \\ 
0.86 & 0.12 \\ 
0.87 & 0.12 \\ 
0.87 & 0.13 \\ 
0.88 & 0.13 \\ 
0.88 & 0.14 \\ 
0.89 & 0.14 \\ 
0.90 & 0.15 \\ 
0.91 & 0.16 \\ 
0.91 & 0.17 \\ 
0.92 & 0.17 \\ 
0.92 & 0.18 \\ 
0.93 & 0.18 \\ 
0.93 & 0.19 \\ 
0.94 & 0.20 \\ 
0.94 & 0.21 \\ 
0.95 & 0.21 \\ 
0.95 & 0.22 \\ 
0.95 & 0.23 \\ 
0.96 & 0.23 \\ 
0.96 & 0.24 \\ 
0.96 & 0.25 \\ 
0.97 & 0.26 \\ 
0.97 & 0.27 \\ 
0.97 & 0.28 \\ 
0.97 & 0.29 \\ 
0.98 & 0.29 \\ 
0.98 & 0.30 \\ 
0.98 & 0.31 \\ 
0.98 & 0.32 \\ 
0.98 & 0.33 \\ 
0.98 & 0.34 \\ 
0.98 & 0.35 \\ 
0.99 & 0.35 \\ 
0.99 & 0.36 \\ 
0.99 & 0.37 \\ 
0.99 & 0.38 \\ 
0.99 & 0.39 \\ 
0.99 & 0.40 \\ 
0.99 & 0.41 \\ 
0.99 & 0.42 \\ 
0.99 & 0.43 \\ 
0.99 & 0.44 \\ 
0.99 & 0.45 \\ 
0.99 & 0.46 \\ 
0.99 & 0.47 \\ 
0.99 & 0.48 \\ 
1.00 & 0.49 \\ 
1.00 & 0.50 \\ 
1.00 & 0.51 \\ 
1.00 & 0.52 \\ 
1.00 & 0.53 \\ 
1.00 & 0.54 \\ 
1.00 & 0.55 \\ 
1.00 & 0.56 \\ 
1.00 & 0.57 \\ 
1.00 & 0.58 \\ 
1.00 & 0.59 \\ 
1.00 & 0.60 \\ 
1.00 & 0.61 \\ 
1.00 & 0.62 \\ 
1.00 & 0.63 \\ 
1.00 & 0.64 \\ 
1.00 & 0.65 \\ 
1.00 & 0.66 \\ 
1.00 & 0.67 \\ 
1.00 & 0.68 \\ 
1.00 & 0.69 \\ 
1.00 & 0.70 \\ 
1.00 & 0.71 \\ 
1.00 & 0.72 \\ 
1.00 & 0.73 \\ 
1.00 & 0.74 \\ 
1.00 & 0.75 \\ 
1.00 & 0.76 \\ 
1.00 & 0.77 \\ 
1.00 & 0.78 \\ 
1.00 & 0.79 \\ 
1.00 & 0.80 \\ 
1.00 & 0.81 \\ 
1.00 & 0.82 \\ 
1.00 & 0.83 \\ 
1.00 & 0.84 \\ 
1.00 & 0.85 \\ 
1.00 & 0.86 \\ 
1.00 & 0.87 \\ 
1.00 & 0.88 \\ 
1.00 & 0.89 \\ 
1.00 & 0.90 \\ 
1.00 & 0.91 \\ 
1.00 & 0.92 \\ 
1.00 & 0.93 \\ 
1.00 & 0.94 \\ 
1.00 & 0.95 \\ 
1.00 & 0.96 \\ 
1.00 & 0.97 \\ 
1.00 & 0.98 \\ 
1.00 & 0.99 \\ 
1.00 & 1.00 \\ 
}\cfdataone

\pgfplotstableread[row sep=\\,col sep=&]{
xa & ya \\
0.15 & 0.00 \\ 
0.20 & 0.00 \\ 
0.26 & 0.01 \\ 
0.29 & 0.01 \\ 
0.33 & 0.01 \\ 
0.36 & 0.01 \\ 
0.38 & 0.02 \\ 
0.40 & 0.02 \\ 
0.42 & 0.02 \\ 
0.44 & 0.02 \\ 
0.45 & 0.02 \\ 
0.46 & 0.03 \\ 
0.47 & 0.03 \\ 
0.48 & 0.03 \\ 
0.49 & 0.03 \\ 
0.50 & 0.03 \\ 
0.51 & 0.03 \\ 
0.52 & 0.04 \\ 
0.53 & 0.04 \\ 
0.54 & 0.04 \\ 
0.55 & 0.04 \\ 
0.56 & 0.05 \\ 
0.57 & 0.05 \\ 
0.58 & 0.05 \\ 
0.59 & 0.05 \\ 
0.60 & 0.06 \\ 
0.61 & 0.06 \\ 
0.62 & 0.06 \\ 
0.62 & 0.07 \\ 
0.63 & 0.07 \\ 
0.64 & 0.07 \\ 
0.65 & 0.07 \\ 
0.65 & 0.08 \\ 
0.66 & 0.08 \\ 
0.67 & 0.08 \\ 
0.67 & 0.09 \\ 
0.68 & 0.09 \\ 
0.69 & 0.09 \\ 
0.69 & 0.10 \\ 
0.70 & 0.10 \\ 
0.70 & 0.11 \\ 
0.71 & 0.11 \\ 
0.72 & 0.12 \\ 
0.73 & 0.12 \\ 
0.73 & 0.13 \\ 
0.73 & 0.14 \\ 
0.74 & 0.14 \\ 
0.74 & 0.15 \\ 
0.75 & 0.15 \\ 
0.75 & 0.16 \\ 
0.75 & 0.17 \\ 
0.76 & 0.17 \\ 
0.76 & 0.18 \\ 
0.76 & 0.19 \\ 
0.77 & 0.19 \\ 
0.77 & 0.20 \\ 
0.77 & 0.21 \\ 
0.78 & 0.21 \\ 
0.78 & 0.22 \\ 
0.78 & 0.23 \\ 
0.78 & 0.24 \\ 
0.78 & 0.25 \\ 
0.78 & 0.26 \\ 
0.79 & 0.26 \\ 
0.79 & 0.27 \\ 
0.79 & 0.28 \\ 
0.79 & 0.29 \\ 
0.79 & 0.30 \\ 
0.79 & 0.31 \\ 
0.79 & 0.32 \\ 
0.79 & 0.33 \\ 
0.79 & 0.34 \\ 
0.79 & 0.35 \\ 
0.79 & 0.36 \\ 
0.80 & 0.36 \\ 
0.80 & 0.37 \\ 
0.80 & 0.38 \\ 
0.80 & 0.39 \\ 
0.80 & 0.40 \\ 
0.80 & 0.41 \\ 
0.80 & 0.42 \\ 
0.80 & 0.43 \\ 
0.80 & 0.44 \\ 
0.80 & 0.45 \\ 
0.80 & 0.46 \\ 
0.80 & 0.47 \\ 
0.80 & 0.48 \\ 
0.80 & 0.49 \\ 
0.80 & 0.50 \\ 
0.80 & 0.51 \\ 
0.80 & 0.52 \\ 
0.80 & 0.53 \\ 
0.80 & 0.54 \\ 
0.80 & 0.55 \\ 
0.80 & 0.56 \\ 
0.80 & 0.57 \\ 
0.80 & 0.58 \\ 
0.80 & 0.59 \\ 
0.80 & 0.60 \\ 
0.80 & 0.61 \\ 
0.80 & 0.62 \\ 
0.80 & 0.63 \\ 
0.80 & 0.64 \\ 
0.80 & 0.65 \\ 
0.80 & 0.66 \\ 
0.80 & 0.67 \\ 
0.80 & 0.68 \\ 
0.80 & 0.69 \\ 
0.80 & 0.70 \\ 
0.80 & 0.71 \\ 
0.80 & 0.72 \\ 
0.80 & 0.73 \\ 
0.80 & 0.74 \\ 
0.80 & 0.75 \\ 
0.80 & 0.76 \\ 
0.80 & 0.77 \\ 
0.80 & 0.78 \\ 
0.80 & 0.79 \\ 
0.80 & 0.80 \\ 
}\cfdatatwo

\pgfplotstableread[row sep=\\,col sep=&]{
xa & ya \\
0 & 1 \\
1 & 1\\
}\dummydata
\centering
\newcommand\dottedcircle{\raisebox{-.1em}{\tikz \draw [line cap=round, line width=0.2ex, dash pattern=on 0pt off 0.5ex] (0,0) circle [radius=0.79ex];}}
%\resizebox{.03\textwidth}{!}{%
%\vspace{-2cm}
\begin{tikzpicture}
    [trim left=9cm,
     trim right=0cm,
     scale=1,
     mycirc/.style={circle,solid,fill=white,draw=black,inner sep=0pt,minimum size=4pt},
     mycirctwo/.style={circle,solid,fill=black,draw=black,inner sep=0pt,minimum size=4pt},
     mydiamond/.style={diamond,solid,fill=white,draw=black,inner sep=0pt,minimum size=4pt},
     graysquare/.style={square*,solid,fill=gray!0.1,draw=gray!0.1,inner sep=0pt,minimum size=4pt},
     every pin/.style = {%pin distance=2mm, 
                font=\scriptsize, inner sep=1pt},
    PNtwo/.style args = {#1/#2}{mycirctwo, pin=#1:#2}
     ]
    \begin{axis}[
    xshift=-3.5cm,
    yshift=1.5cm,
    title={},
    %scale=1.2,
    width=12cm,
    height=9cm,
    ymin=-1,ymax=1,xmin=-1,xmax=0.75,
    ytick={0,1},xtick={0,1},
    ymajorgrids=false,
    yminorgrids=false,
    every axis plot post/.style={/pgf/number format/fixed},        
    axis x line*=bottom,
    axis y line*=left,
    hide y axis,
    hide x axis,
    xtick style={draw=none},
    ytick style={draw=none},
    %xtick label style={draw=none},
    %axis x line style={draw=none},
    %ymode=log,
    ]
    \path[name path=axis1b] (axis cs:0,0) -- (axis cs:0.65,0);
    \path[name path=axis2b] (axis cs:0,0.65) -- (axis cs:0.5,0.65);
    %\draw [->] (0,0) -- (0.55,0) node {{\small Demographic Fairness \\ \small ($\tau$=1)}};
    \draw (0,0) -- (0.6,0);
    \draw (0,0.5) -- (0.6,0.5);
    \draw (0.6,0) -- (0.6,0.5);
    %\draw [->] (0,0) -- (0,0.55) node [midway, above, rotate=90,text width=3cm, align=center] {\small Linguistic Fairness \\ \small ($\tau$=0)};
    \draw (0,0) -- (0,0.5);
    %\node[mycirc, label=above:{Ideal}] at (axis cs:1,1) {};
    \node[label={Inflection}] at (axis cs:0.22,0.34) {};
    %\node[label={Inflection}] at (axis cs:0.16,0.24) {};
    \node[label=below:{0}] at (axis cs:0,0.03) {};
    \node[label=below:{0.5}] at (axis cs:0.5,0.03) {};
    \node[label=left:{0.1}] at (axis cs:0.03,0.5) {};
    \addplot[name path=f, domain=0:0.6,black] {x^5};
    \addplot [thick,color=gray, fill=gray, fill opacity=0.1]
    fill between[of=f and axis1b,soft clip={domain=0:0.6},];
    %\addplot[name path=g, domain=0:0.037,black] {x^.16};
    %\addplot [thick,color=gray, fill=gray, fill opacity=0.1,]
    %fill between[of=axis2b and g,soft clip={domain=0:0.037},];
    % My stuff
    \node[mycirctwo, pin={[pin distance=2mm]90:{\small 2020}}] at (axis cs:0.564,0.26) {}; 
    \node[mycirctwo, pin={[pin distance=2mm]30:{\small 2019}}] at (axis cs:0.54,0.18) {};
    \node[mycirctwo, pin={[pin distance=2mm]150:{\small 2018}}] at (axis cs:0.54,0.16) {};
    \node[mycirctwo, pin={[pin distance=2mm]180:{\small 2017}}] at (axis cs:0.497,0.11) {};
    \node[mycirctwo, pin={[pin distance=2mm]90:{\small 2016}}] at (axis cs:0.16,0.03) {};
    \end{axis}
    \iffalse
    \begin{axis}[
    xshift=-1cm,
    yshift=1.5cm,
    title={},
    %scale=1.2,
    width=12cm,
    height=9cm,
    ymin=-1,ymax=1,xmin=-1,xmax=0.75,
    ytick={0,1},xtick={0,1},
    ymajorgrids=false,
    yminorgrids=false,
    every axis plot post/.style={/pgf/number format/fixed},        
    axis x line*=bottom,
    axis y line*=left,
    hide y axis,
    hide x axis,
    xtick style={draw=none},
    ytick style={draw=none},
    %xtick label style={draw=none},
    %axis x line style={draw=none},
    %ymode=log,
    ]
    \path[name path=axis1b] (axis cs:0,0) -- (axis cs:0.65,0);
    \path[name path=axis2b] (axis cs:0,0.65) -- (axis cs:0.5,0.65);
    %\draw [->] (0,0) -- (0.55,0) node {{\small Demographic Fairness \\ \small ($\tau$=1)}};
    \draw (0,0) -- (0.6,0);
    \draw (0,0.5) -- (0.6,0.5);
    \draw (0.6,0) -- (0.6,0.5);
    %\draw [->] (0,0) -- (0,0.55) node [midway, above, rotate=90,text width=3cm, align=center] {\small Linguistic Fairness \\ \small ($\tau$=0)};
    \draw (0,0) -- (0,0.5);
    %\node[mycirc, label=above:{Ideal}] at (axis cs:1,1) {};
    \node[label={Inflection}] at (axis cs:0.22,0.34) {};
    %\node[label={Inflection}] at (axis cs:0.16,0.24) {};
    \node[label=below:{0}] at (axis cs:0,0.03) {};
    \node[label=below:{0.5}] at (axis cs:0.5,0.03) {};
    \node[label=left:{0.1}] at (axis cs:0.03,0.5) {};
    \addplot[name path=f, domain=0:0.6,black] {x^5};
    \addplot [thick,color=gray, fill=gray, fill opacity=0.1]
    fill between[of=f and axis1b,soft clip={domain=0:0.6},];
    %\addplot[name path=g, domain=0:0.037,black] {x^.16};
    %\addplot [thick,color=gray, fill=gray, fill opacity=0.1,]
    %fill between[of=axis2b and g,soft clip={domain=0:0.037},];
    % My stuff
    \node[mycirctwo, pin={[pin distance=2mm]90:{\small 2020}}] at (axis cs:0.564,0.26) {}; 
    \node[mycirctwo, pin={[pin distance=2mm]30:{\small 2019}}] at (axis cs:0.54,0.18) {};
    \node[mycirctwo, pin={[pin distance=2mm]150:{\small 2018}}] at (axis cs:0.54,0.16) {};
    \node[mycirctwo, pin={[pin distance=2mm]180:{\small 2017}}] at (axis cs:0.497,0.11) {};
    \node[mycirctwo, pin={[pin distance=2mm]90:{\small 2016}}] at (axis cs:0.16,0.03) {};
    \end{axis}
    \fi
    \begin{axis}[
    xshift=-5.5cm,
    yshift=-1cm,
    title={},
    %scale=1.2,
    width=12cm,
    height=9cm,
    ymin=-1,ymax=1,xmin=-1,xmax=0.75,
    ytick={0,1},xtick={0,1},
    ymajorgrids=false,
    yminorgrids=false,
    every axis plot post/.style={/pgf/number format/fixed},        
    axis x line*=bottom,
    axis y line*=left,
    hide y axis,
    hide x axis,
    xtick style={draw=none},
    ytick style={draw=none},
    %xtick label style={draw=none},
    %axis x line style={draw=none},
    %ymode=log,
    ]
    \path[name path=axis1b] (axis cs:0,0) -- (axis cs:0.65,0);
    \path[name path=axis2b] (axis cs:0,0.65) -- (axis cs:0.5,0.65);
    %\draw [->] (0,0) -- (0.55,0) node {{\small Demographic Fairness \\ \small ($\tau$=1)}};
    \draw (0,0) -- (0.6,0);
    \draw (0,0.5) -- (0.6,0.5);
    \draw (0.6,0) -- (0.6,0.5);
    %\draw [->] (0,0) -- (0,0.55) node [midway, above, rotate=90,text width=3cm, align=center] {\small Linguistic Fairness \\ \small ($\tau$=0)};
    \draw (0,0) -- (0,0.5);
    %\node[mycirc, label=above:{Ideal}] at (axis cs:1,1) {};
    \node[label={MT from English}] at (axis cs:0.22,0.34) {};
    %\node[label={Inflection}] at (axis cs:0.16,0.24) {};
    \node[label=below:{0}] at (axis cs:0,0.03) {};
    \node[label=below:{0.5}] at (axis cs:0.5,0.03) {};
    \node[label=left:{0.1}] at (axis cs:0.03,0.5) {};
    \addplot[name path=f, domain=0:0.6,black] {x^5};
    \addplot [thick,color=gray, fill=gray, fill opacity=0.1]
    fill between[of=f and axis1b,soft clip={domain=0:0.6},];
    %\addplot[name path=g, domain=0:0.037,black] {x^.16};
    %\addplot [thick,color=gray, fill=gray, fill opacity=0.1,]
    %fill between[of=axis2b and g,soft clip={domain=0:0.037},];
    % My stuff
    \node[mycirctwo, pin={[pin distance=3mm]60:{\small 2021}}] at (axis cs:0.25,0.028) {}; 
    \node[mycirctwo, pin={[pin distance=2mm]0:{\small 2020}}] at (axis cs:0.23,0.024) {}; 
    \node[mycirctwo, pin={[pin distance=1mm]60:{\small 2019}}] at (axis cs:0.195,0.012) {};
    \node[mycirctwo, pin={[pin distance=4mm]90:{\small 2018}}] at (axis cs:0.17,0.006) {};
    \node[mycirctwo, pin={[pin distance=1mm]90:{\small 2017}}] at (axis cs:0.08,0.004) {};
    \node[mycirctwo, pin={[pin distance=2mm]165:{\small 2016}}] at (axis cs:0.077,0.003) {};
    \end{axis}
    \begin{axis}[
    xshift=-1cm,
    yshift=-1cm,
    title={},
    %scale=1.2,
    width=12cm,
    height=9cm,
    ymin=-1,ymax=1,xmin=-1,xmax=0.75,
    ytick={0,1},xtick={0,1},
    ymajorgrids=false,
    yminorgrids=false,
    every axis plot post/.style={/pgf/number format/fixed},        
    axis x line*=bottom,
    axis y line*=left,
    hide y axis,
    hide x axis,
    xtick style={draw=none},
    ytick style={draw=none},
    %xtick label style={draw=none},
    %axis x line style={draw=none},
    %ymode=log,
    ]
    \path[name path=axis1b] (axis cs:0,0) -- (axis cs:0.65,0);
    \path[name path=axis2b] (axis cs:0,0.65) -- (axis cs:0.5,0.65);
    %\draw [->] (0,0) -- (0.55,0) node {{\small Demographic Fairness \\ \small ($\tau$=1)}};
    \draw (0,0) -- (0.6,0);
    \draw (0,0.5) -- (0.6,0.5);
    \draw (0.6,0) -- (0.6,0.5);
    %\draw [->] (0,0) -- (0,0.55) node [midway, above, rotate=90,text width=3cm, align=center] {\small Linguistic Fairness \\ \small ($\tau$=0)};
    \draw (0,0) -- (0,0.5);
    %\node[mycirc, label=above:{Ideal}] at (axis cs:1,1) {};
    \node[label={MT to English}] at (axis cs:0.22,0.34) {};
    %\node[label={Inflection}] at (axis cs:0.16,0.24) {};
    \node[label=below:{0}] at (axis cs:0,0.03) {};
    \node[label=below:{0.5}] at (axis cs:0.5,0.03) {};
    \node[label=left:{0.1}] at (axis cs:0.03,0.5) {};
    \addplot[name path=f, domain=0:0.6,black] {x^5};
    \addplot [thick,color=gray, fill=gray, fill opacity=0.1]
    fill between[of=f and axis1b,soft clip={domain=0:0.6},];
    %\addplot[name path=g, domain=0:0.037,black] {x^.16};
    %\addplot [thick,color=gray, fill=gray, fill opacity=0.1,]
    %fill between[of=axis2b and g,soft clip={domain=0:0.037},];
    % My stuff
    \node[mycirctwo, pin={[pin distance=2mm]0:{\small 2021}}] at (axis cs:0.267,0.035) {}; 
    \node[mycirctwo, pin={[pin distance=4mm]60:{\small 2020}}] at (axis cs:0.258,0.031) {}; 
    \node[mycirctwo, pin={[pin distance=2mm]60:{\small 2019}}] at (axis cs:0.214,0.017) {};
    \node[mycirctwo, pin={[pin distance=4mm]90:{\small 2018}}] at (axis cs:0.168,0.008) {};
    \node[mycirctwo, pin={[pin distance=1mm]90:{\small 2017}}] at (axis cs:0.045,0.003) {};
    \node[mycirctwo, pin={[pin distance=2mm]165:{\small 2016}}] at (axis cs:0.039,0.002) {};
    \end{axis}

\end{tikzpicture}
%}
\vspace{-2.5cm}
\caption{Historical \gn{more detail}}
\label{fig:historical}
%\end{figure}
\end{figure}
